Keyphrase Generation for Scientific Document Retrieval

Sequence-to-sequence models have lead to significant progress in keyphrase generation, but it remains unknown whether they are reliable enough to be beneficial for document retrieval. This study provides empirical evidence that such models can significantly improve retrieval performance, and introduces a new extrinsic evaluation framework that allows for a better understanding of the limitations of keyphrase generation models. Using this framework, we point out and discuss the difficulties encountered with supplementing documents with -- not present in text -- keyphrases, and generalizing models across domains. Our code is available at https://github.com/boudinfl/ir-using-kg

==> tables/ir_per_field.tex <==


\begin{table*}[ht!]
    \centering
    \begin{tabular}{l|ccccr}
        \toprule
        Field & size & title+abstract & + s2s+copy & $\Delta$\\
        \midrule
        1 Electricity, information and control & 15 & 28.08 & 29.58 & +5.4\%\\
        2 Chemistry & 9  & 36.43 & \sign{39.48} & +8.4\%\\
        3 Architecture, civil engineering and landscape gardening & 7  & 28.30 & \sign{32.49} & +14.8\%\\
        4 Biology and agriculture & 10 & 43.21 & \sign{45.34} & +4.9\%\\
        5 Science & 8  & 38.03 & 38.73 & +1.8\%\\
        6 Engineering & 5  & 47.24 & \sign{53.31} & +12.8\%\\
        7 Medicine and dentistry & 17 & 34.58 & 35.83 & +3.6\%\\
        8 Cultural and social science &  7 & 17.00 & 18.13 & +6.6\%\\
        \midrule
        all & 49 & 31.93 & \sign{33.56} & +5.1\%\\
        \bottomrule
    \end{tabular}
    \caption{BM25+RM3}
    \label{tab:per_field}
\end{table*}

